The Paradox of Information Access: Growing Isolation in the Age of Sharing

Modern online media, such as Twitter, Instagram, and YouTube, enable anyone to become an information producer and to offer online content for potentially global consumption. By increasing the amount of globally accessible real-time information, today's ubiquitous producers contribute to a world, where an individual consumes vanishingly smaller fractions of all produced content. In general, consumers preferentially select information that closely matches their individual views and values. The bias inherent in such selection is further magnified by today's information curation services that maximize user engagement (and thus service revenue) by filtering new content in accordance with observed consumer preferences. Consequently, individuals get exposed to increasingly narrower bands of the ideology spectrum. Societies get fragmented into increasingly ideologically isolated enclaves. These enclaves (or echo-chambers) then become vulnerable to misinformation spread, which in turn further magnifies polarization and bias. We call this dynamic the paradox of information access; a growing ideological fragmentation in the age of sharing. This article describes the technical, economic, and socio-cognitive contributors to this paradox, and explores research directions towards its mitigation.

==> 011-Model.tex <==
\section{A Simple Belief Model}
In this section, we present a simple stylized analytic model of producers, consumers, and curators in the information landscape just described, as a means to understand the emerging co-evolution dynamics of human beliefs and information flow in the age of overload. Simulation of this model confirms the emergence of the paradox described: namely, ideological fragmentation and isolation as ubiquitous sharing causes total information volume to significantly exceed the individuals' cognitive capacity. 

We model individuals in a society as agents.
Let \(\mathbf{x}_{i, t} \in \mathbb{R}^K\) denote the position of agent \(a_i~(i=1, 2,\cdots, n)\) in a K-dimensional ``belief space'' at time \(t\). It reflects the agent's belief at time \(t\). We assume the origin point of the belief space as neutrality. Departures from the origin represent bias towards specific beliefs, where {\em direction\/} encodes the nature of the belief (e.g., liberal versus conservative) and {\em magnitude\/} represents the degree to which the belief is upheld, where $0$ is neutral and $1$ is the far extreme. Hence,
\(0 \leq \|\mathbf{x}_{i, t}\| \leq 1\) reflects how extreme agent \(a_i\)'s belief is. Let \(\mathbf{X_t}\) denote the entire population of \(n\) agents. Similarly, we define the set of documents, $\mathbf{Y}_t$, where $\mathbf{y}_{j,t} \in \mathbf{Y}_t$ represents the belief espoused by the $j$th document, produced at time $t$.

\begin{comment}
A \emph{producer} function takes, as input, the bias of sources \(\mathbf{X}_{t}\) and generates the population of content \(\mathbf{Y}_t\) that contains \(n'\) new positions generated at time \(t\). Hence:
\begin{equation}
    \text{producer}(\mathbf{X}_t) \rightarrow \mathbf{Y}_t
\end{equation}

A \emph{curator} function takes as input the belief of each agent \(a_i\) and the recent content \(\mathbf{Y}_t\), then returns a subset \(\mathbf{Y}^{(i)}_t \subseteq \mathbf{Y}_t\) to show to the agent. The subset \(\mathbf{Y}^{(i)}_t\) represents the content that agent \(a_i\) can see.
% \begin{equation}
%     \text{curator}(\mathbf{Y}_t, i) \rightarrow \mathbf{Y}^{(i)}_t
% \end{equation}

\begin{equation}
    \text{curator}(\mathbf{Y}_t, \mathbf{x}_{i, t}) \rightarrow \mathbf{Y}^{(i)}_t
\end{equation}

A \emph{consumer} function takes an agent's position \(\mathbf{x}_{i, t}\), its visible content \(\mathbf{Y}^{(i)}_t\), and returns a new position for the agent, \(\mathbf{x}_{i, t+1}\). It reflects the effect of the visible content on the agent's belief.
\begin{equation}
    \text{consumer}(\mathbf{Y}^{(i)}_t, \mathbf{x}_{i, t}) \rightarrow \mathbf{x}_{i, t+1}
\end{equation}

Next, we inject some of features of modern information flow into the above model.
\end{comment}

\subsection{Democratized Production}

We assume that, on a fully democratized medium, everyone is a content producer who propagates its current belief. Thus:
\begin{equation}
    \mathbf{Y}_t = \mathbf{X}_t
\end{equation}

\subsection{Engagement-maximizing Curation}

We assume that in order to maximize engagement, a content curator recommends content set $\mathbf{C}^{(i)}_t$, to recipient $a_i$,  that matches the intended recipient's belief. For each recipient, assume that a visibility radius \(r_i\) limits how ideologically distant the content they engage with can be. Thus:
\begin{equation}
    \mathbf{C}^{(i)}_t = \{\mathbf{y}_j | \mathbf{y}_j \in \mathbf{Y}_t,  \|\mathbf{x}_{i,t} - \mathbf{y}_{j}\| \leq r_i\}
    \label{eq:curator}
\end{equation}

\subsection{Capacity-constrained Consumption}
Since consumers do not have unlimited cognitive capacity, we imagine that consumers can only process $k$ pieces of information. We distinguish between biased consumers who preferentially read content that meets their belief, and those consumers who sample content more uniformly. We call the former {\em biased\/} and the latter {\em uniform\/} consumers, respectively.

{\em Biased consumer:\/}
Such an agent reads
the k-nearest neighbors to the agent's position. Let set, $\mathbf{Y}^{(i)}_t$, represent the content browsed by consumer $a_i$. It can be described as follows:
\begin{equation}
    \mathbf{Y}^{(i)}_t = \{\mathbf{y}_j | \mathbf{y}_j \in \mathrm{KNN}(\mathbf{C}^{(i)}_t, \mathbf{x}_{i,t}), \mathbf{y}_j \in \mathbf{C}^{(i)}_t\}
\end{equation}

{\em Uniform consumer:\/}
Such an agent uniformly samples $k$ content pieces from those returned by the curator, according to Equation~(\ref{eq:curator}).

\subsection{Belief Update}

Consistently with prior literature~\cite{fiske1980attention,shoemaker1996hardwired,lamberson2018model,varshney2019must}, 
We assume that, of the content consumed by an agent, more outlying news leave a deeper impression. We define an \emph{influence} function, $\eta$, to reflect such a tendency, giving more influence to more outlying news:
\begin{equation}
    \eta(\mathbf{y}_{j}) \propto \|\mathbf{y}_{j}\|
\end{equation}

The updated position of the agent \(i\) is the weighted average (\(0<\alpha < 1\)) of its current position and the weighted normalized positions of content it consumes, \(\mathbf{Y}^{(i)}_t\):

% \begin{equation}
%     \mathbf{x}_{i,t+1} = \alpha_0 \mathbf{x}_{i,t} + \alpha_1 \sum_{\mathbf{y}_j \in \mathbf{Y}^{(i)}_t} \eta(\mathbf{y}_{j}) \mathbf{y}_{j}
% \end{equation}


\begin{equation}
    \mathbf{x}_{i,t+1} = \alpha \cdot \mathbf{x}_{i,t} + (1-\alpha)\cdot  \frac{\sum_{\mathbf{y}_j \in \mathbf{Y}^{(i)}_t} \eta(\mathbf{y}_{j}) \mathbf{y}_{j}}{\sum_{\mathbf{y}_j \in \mathbf{Y}^{(i)}_t} \eta(\mathbf{y}_{j})}
\end{equation}

\subsection{Model Simulation Results}
The above model can be simulated to describe the evolution of belief in societies with omnipresent content producers and consumer-driven curation. 

\textcolor{red}{Jinyang will insert simulation results here.}

The rest of this paper reviews solutions that may break the vicious cycles described above, by addressing some of the challenges in  Figure~\ref{fig:info}.
A key ingredient of the solution is to reduce channel distortion introduced in both {\em content visibility\/} and {\em provenance\/}, as well as increase the difficulty of inserting disinformation. 
These solutions are described next.


 %Since we cannot infringe on the consumers' freedom to act as they choose, we primarily consider solutions that target producers and curators in the two sections below.


==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> Textstyle.tex <==

\subsection{Text Style and Author Bias Detection}

Another important aspect is to model author style. Syntactic, lexical, and semantic features can be combined to model the source styles and investigate hierarchical models based on topic modeling, context, and cultures. 

New, reliable truth-finding methods need to be developed with confidence estimation and source profiling by improving state-of-the-art information extraction modules in two ways. 
%
First, attention should be on the specific coherent knowledge suggested by the cross-source evidence. Second, incorporating context, such as a source's profile (e.\,g., political stance, localization, origin, cultural background, etc.) by analysis of historical data to improve future predictions. For example, if the source was previously arrested in an anti-government protest, they are more likely to have anti-government views. Compared to previous work on stance detection~\cite{Hanselowski2018}, each dimension of source profiling should be associated with certain issues by automatic issue detection. 

In order to detect source bias and stance, fine-grained discourse analysis is required by organizing each document as a hierarchical, structural, discourse-level dependency tree~\cite{Karimi2019}. In contrast to previous work~\cite{Hanselowski2018} that only represents words and sentences, a comprehensive framework needs to incorporate knowledge elements from our information extraction algorithms mentioned above, human value detection~\cite{Mooijman2018}, and salient topical keywords into determining 21 types of fine-grained relations~\cite{hong2016building}. This will result in meta-paths to trace how styles and topics shift and rumors propagate.

\begin{figure}[!htb]
    \includegraphics[width=\linewidth]{fig/truthfinding}
    \caption{Multi-dimensional truth finding.}
    \label{fig:truthfinding}
\end{figure}

Furthermore, one may develop a continuous learning component to discover novel entities and events; update their profiles over time; and rank their discriminative characteristics for profile construction.  It will update knowledge by self-boosting, self-selection, and self-correction.


Finally, the constructed KG can be embedded in a richer and wider context, and each knowledge element can be connected with its source (Figure~\ref{fig:truthfinding}). The unified KG will contain the time and location of each event, and source reliability expectations
(e.\,g., an FBI report is more reliable than an anonymous post on Reddit). 
Our previous work on unsupervised truth-finding framework can be used to  authenticate KG elements and assertions. Each knowledge element’s credibility score is initialized by combining the confidence values produced from multimedia information extraction algorithms. Then our Tri-HITS algorithm~\cite{Huang2012,Ma2015,Yu2014,Zhi2015} can be extended to propagate credibility scores iteratively across multiple dimensions and update across co-linked dimensions based on mutual reinforcement. \heng{Tarek, do you want to mention your more recent truth finding algorithms here?}

